The Shifting Sands of Motivation: Revisiting What Drives Contributors in Open Source

Open Source Software (OSS) has changed drastically over the last decade, with OSS projects now producing a large ecosystem of popular products, involving industry participation, and providing professional career opportunities. But our field's understanding of what motivates people to contribute to OSS is still fundamentally grounded in studies from the early 2000s. With the changed landscape of OSS, it is very likely that motivations to join OSS have also evolved. Through a survey of 242 OSS contributors, we investigate shifts in motivation from three perspectives: (1) the impact of the new OSS landscape, (2) the impact of individuals' personal growth as they become part of OSS communities, and (3) the impact of differences in individuals' demographics. Our results show that some motivations related to social aspects and reputation increased in frequency and that some intrinsic and internalized motivations, such as learning and intellectual stimulation, are still highly relevant. We also found that contributing to OSS often transforms extrinsic motivations to intrinsic, and that while experienced contributors often shift toward altruism, novices often shift toward career, fun, kinship, and learning. OSS projects can leverage our results to revisit current strategies to attract and retain contributors, and researchers and tool builders can better support the design of new studies and tools to engage and support OSS development.

==> Tables/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> Tables/Tables/codes.tex <==
\begin{table*}[htb]
\centering
%\scriptsize
\caption{Regions, Quadrants and Dimensions of Dries et al.'s   model \cite{dries2008career} that we classified the success meanings cited by the Interviewed Participants}
\label{tab:codes}
\footnotesize
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l|l|l|r|r}
\hline
\rowcolor{gray!35}\multicolumn{2}{c|}{ } & & \multicolumn{1}{|c|}{\textbf{\# Interviews}} & \multicolumn{1}{c}{\textbf{\# Survey }} \\
\rowcolor{gray!35}&\textbf{Region} & \textbf{Participants' IDs (Interviews)}& \multicolumn{1}{c|}{\textbf{(total: 27)}} & \multicolumn{1}{c}{\textbf{(total: 193)}} \\\hline\hline

\multirow{4}{*}{Q1}
& Cooperation            &  P2, P3, P4, P5, P7, P8, P13, P15, P17, P20, P21 & 11 & 19 \\\cline{2-5}
& Perceived Contribution & P5, P6, P9, P11, P17, P18, P21, P22, P25         & 9  & 54\\ \cline{2-5}
& Recognition            & P1, P9, P13, P22, P23, P25                       & 6  & 29 \\  \cline{2-5}
\rowcolor{gray!10}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region from Q1}& \textbf{19} & \textbf{90}\\\hline\hline
 
 
\multirow{4}{*}{Q2}
& Advancement           & P1, P10, P12, P16, P20, P21, P22, P23, P24 & 8 & 77\\\cline{2-5}
& Performance           & P4                                         & 1 & 0 \\\cline{2-5}
& Factual Contribution  & P2, P6, P12, P14, P18, P19, P20, P21       & 8 & 9\\\cline{2-5}
\rowcolor{gray!10}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region from Q2}& \textbf{15} & \textbf{84} \\\hline\hline

\multirow{3}{*}{Q3}
& Self-Development  & P7, P16, P18, P19, P20, P21, P24 & 7  & 19 \\\cline{2-5}
& Creativity        & P10                              & 1  & 2  \\\cline{2-5}
\rowcolor{gray!10}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region from Q3}& \textbf{8} & \textbf{21} \\\hline\hline

 
\multirow{3}{*}{Q4} 
& Satisfaction  & P1, P5, P10, P16, P21 & 5  & 13 \\ \cline{2-5}
& Security      & P19, P24              & 2  & 17 \\ \cline{2-5}
\rowcolor{gray!10}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region from Q4}&  \textbf{7} & \textbf{30} \\\hline\hline

\end{tabular}
}

\resizebox{0.80\textwidth}{!}{%
\tiny
\begin{tabular}{r}
\textbf{Q1}: Inter-Personal x Affect; \textbf{Q2}: Inter-Personal x Achievement; \textbf{Q3}: Intra-Personal x Achievement; \textbf{Q4}: Intra-Personal x Affect\\
The total per quadrant is not the sum of the regions since the participants often provided an answer that was categorized into \textbf{more than one region}.
\end{tabular}
}


\end{table*}

==> Tables/Tables/codes_by_role.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htb]
\centering
\caption{Quadrants and Regions cited by the Interview's Participants who play roles as coders and non-coders}
\label{tab:codes_by_role}
\footnotesize
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Quadrant}                     & \multirow{2}{*}{Region} & \multicolumn{2}{c|}{Participants ID}            \\ \cline{3-4} 
 &             & Coders (12)               & Non-Coders (15)                \\ \hline
\multirow{2}{*}{Intra-Personal x Affect}      & Satisfaction            & P5, P21                    & P1, P10, P16, P26      \\ \cline{2-4} 
 & Security    & P19, P24             &                           \\ \hline
\multirow{2}{*}{Intra-Personal x Achievement} & Self-Development        & P7, P18, P19, P20, P21, P24 & P12, P16          \\ \cline{2-4} 
 & Creativity  &                      & P10                       \\ \hline
\multirow{3}{*}{Inter-Personal x Affect}      & Perceived Contribution  & P5, P6, P18, P21, P25       & P22, P9, P11, P17 \\ \cline{2-4} 
 & Cooperation & P2, P5, P7, P20, P21 & P3, P4, P8, P13, P15, P17 \\ \cline{2-4} 
 & Recognition & P23, P25, P27             & P1, P9, P13, P22          \\ \hline
\multirow{3}{*}{Inter-Personal x Achievement} & Factual Contribution    & P2, P6, P18, P19, P20, P21  & P12, P14          \\ \cline{2-4} 
 & Advancement & P20, P21, P23, P24, P27   & P1, P10, P16, P22         \\ \cline{2-4} 
 & Performance &                      & P4                        \\ \hline
\end{tabular}
\end{table*}

==> Tables/Tables/codes_survey.tex <==
\begin{table*}[htb]
\centering
\caption{Quadrants and Regions of Dries et al.'s model \cite{dries2008career} that we classified the success meanings cited by the Survey's Respondents per role, gender and financial relation with OSS}
\label{tab:codes_survey}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
\hline
  \multicolumn{1}{c}{\multirow{3}{*}{}} &
%  \multirow{3}{*}{\textbf{Region}} &
  &
  \multicolumn{4}{c|}{\textbf{Role}} &
  \multicolumn{6}{c|}{\textbf{Gender}} &
  \multicolumn{6}{c|}{\textbf{Financial Relation with OSS}}&
  \multicolumn{2}{c}{}  \\ 
  \cline{3-18} 
  \multicolumn{1}{c}{}&
  \multicolumn{1}{c|}{\textbf{Region}} &
  \multicolumn{2}{c|}{Coders} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Non\\ Coders\end{tabular}} &
  \multicolumn{2}{c|}{Men} &
  \multicolumn{2}{c|}{Women} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Non\\ Binary\end{tabular}} &
  \multicolumn{2}{c|}{Paid} &
  \multicolumn{2}{c|}{Unpaid} &
  \multicolumn{2}{c|}{\begin{tabular}[c|]{@{}c@{}}Partially\\Paid\end{tabular}} 
  &
  \multicolumn{2}{c}{\textbf{Total} }\\ \cline{3-20} 
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c|}{}&
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% &
  \# &
  \% \\ \hline\hline

\multirow{3}{*}{Q1} &

Cooperation &
  14 &
  8.5\% &
  5 &
  16.7\% &
  16 &
  9.7\% &
  0 &
  0.0\% &
  2 &
  100.0\% &
  5 &
  13.9\% &
  10 &
  7.3\% &
  0 &
  0.0\% 
    &
  19&
  8.0\%
  \\ \cline{2-20} 

 &

  Perceived Contr. &
  48 &
  29.5\% &
  6 &
  20.0\% &
  50 &
  30.3\% &
  2 &
  12.5\% &
  0 &
  0.0\% &
  10 &
  27.8\% &
  40 &
  29.2\% &
  3 &
  18.8\% 
    &
  54&
  22.6\%
  \\ \cline{2-20} 

 &
  
  Recognition &
  25 &
  15.3\% &
  4 &
  13.3\% &
  24 &
  14.6\% &
  4 &
  25.0\% &
  0 &
  0.0\% &
  5 &
  13.9\% &
  21 &
  15.3\% &
  3 &
  18.8\% 
    &
  29&
  12.1\%
\\ \hline
\multirow{2}{*}{Q2} &
  Advancement &
  8 &
  4.9\% &
  1 &
  3.3\% &
  8 &
  4.9\% &
  1 &
  6.3\% &
  0 &
  0.0\% &
  1 &
  6.7\% &
  4 &
  2.9\% &
  2 &
  12.5\% 
    &
  9&
  3.8\%
  \\ \cline{2-20} 

 &
 
  Performance &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  0 &
  0.0\% 
    &
  0&
  0.0\%
  \\ \cline{2-20} 
 
 &
 
  Factual Contr. &
  65 &
  39.9\% &
  12 &
  40.0\% &
  63 &
  38.2\% &
  7 &
  43.8\% &
  1 &
  50.0\% &
  15 &
  41.7\% &
  54 &
  39.4\% &
  6 &
  37.5\% 
    &
  77&
  32.2\%
\\ \hline

\multirow{2}{*}{Q3} &
  Self-Development &
  15 &
  9.2\% &
  4 &
  13.3\% &
  17 &
  10.3\% &
  1 &
  6.3\% &
  0 &
  0.0\% &
  2 &
  5.6\% &
  14 &
  10.2\% &
  2 &
  12.6\% 
  &
  19&
  8.0\%
  \\ \cline{2-20} 
 &
  Creativity &
  1 &
  0.6\% &
  1 &
  3.3\% &
  2 &
  1.2\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  1 &
  2.8\% &
  1 &
  0.7\% &
  0 &
  0.0\% 
    &
  2&
  0.9\%
\\ \hline

\multirow{2}{*}{Q4} &
  Satisfaction &
  10 &
  6.1\% &
  3 &
  10.0\% &
  10 &
  6.0\% &
  1 &
  12.5\% &
  0 &
  0.0\% &
  0 &
  0.0\% &
  11 &
  8.0\% &
  1 &
  6.3\% 
  &
  13&
  5.4\%
  \\ \cline{2-20} 
 &
  Security &
  17 &
  10.4\% &
  0 &
  0.0\% &
  15 &
  9.0\% &
  2 &
  6.3\% &
  0 &
  0.0\% &
  3 &
  8.3\% &
  9 &
  6.6\% &
  5 &
  31.3\% 
  &
  17&
  7.1\%
  \\ \hline


\multicolumn{2}{r|}{Total unique resp.} &
  163 &
   &
  30 &
   &
  165 &
   &
  16 &
   &
  2 &
   &
  36 &
   &
  137 &
   &
  16 &
   & 193
  &
   \\ \hline
\end{tabular}
}

\resizebox{\textwidth}{!}{%
\tiny
\begin{tabular}{r}
\textbf{Q1}: Inter-Personal x Affect; \textbf{Q2}: Inter-Personal x Achievement; \textbf{Q3}: Intra-Personal x Achievement; \textbf{Q4}: Intra-Personal x Affect; \\
The sum of each quadrant can differ from the total of unique respondents as people often provided an answer to the open question that was categorized into more than one region. 
\end{tabular}
}

\end{table*}


==> Tables/Tables/demo.tex <==
\begin{table*}[htb]
\centering
\caption{Demographics for the Interview Participants}
\label{tab:demo}
\begin{tabular}{c|c|c|c|c|c}
\hline
\cellcolor{gray!35}\textbf{Participant ID} & \cellcolor{gray!35}\textbf{Gender}        & \cellcolor{gray!35}\textbf{Years in OSS} & \cellcolor{gray!35}\textbf{Main Role}  & \cellcolor{gray!35}\textbf{Recruitment} & \cellcolor{gray!35}\textbf{Interview Mode} \\ \hline
P1  & Woman                  & 6  & OSS Advocate            & OSCON Speaker & In-person       \\ 
P2  & Woman                  & 5  & OSS Coder               & Mature project   & Video-conference \\ 
P3  & Woman                  & 13 & OSS Treasurer           & OSCON Speaker & In-person       \\ 
P4  & Man                    & 9  & OSS System Admin        & OSCON Speaker & In-person       \\ 
P5  & Prefer not to disclose & 7  & OSS Coder               & OSCON Speaker & In-person       \\ 
P6  & Man                    & 5  & OSS Coder               & OSCON Speaker & In-person       \\ 
P7  & Man                    & 12 & OSS Coder               & OSCON Speaker & In-person       \\ 
P8  & Woman                  & 30 & OSS Strategist          & OSCON Speaker & In-person       \\ 
P9  & Man                    & 13 & OSS Advocate            & OSCON Speaker & In-person       \\ 
P10 & Woman                  & 20 & OSS Advocate            & OSCON Speaker & In-person       \\ 
P11 & Woman                  & 20 & OSS Writer              & Snowballing      & Video-conference \\ 
P12 & Woman                  & 20 & OSS Advocate and Writer & OSCON Speaker & In-person       \\ 
P13 & Woman                  & 7  & OSS Advocate            & Mature project   & Video-conference \\ 
P14 & Woman                  & 20 & OSS License Manager     & Mature project   & Video-conference \\ 
P15 & Woman                  & 15 & OSS Advocate            & OSCON Speaker    & In-person       \\ 
P16 & Woman                  & 10 & OSS Advocate            & Snowballing      & Video conference \\ 
P17 & Woman                  & 5  & OSS Project Manager     & OSCON Speaker & In-person       \\ 
P18 & Man                    & 8  & OSS Coder               & Mature project   & Video-conference \\ 
P19 & Man                    & 8  & OSS Coder               & Mature project   & Video-conference \\ 
P20 & Man                    & 5  & OSS Coder               & Mature project   & Video-conference \\ 
P21 & Man                    & 15 & OSS Coder               & Mature project   & Video-conference \\ 
P22 & Man                    & 10 & OSS Advocate            & Mature project   & Video-conference \\ 
P23 & Man                    & 7  & OSS Coder               & Snowballing      & Video-conference \\ 
P24 & Man                    & 20 & OSS Coder               & Mature project   & Video-conference \\ 
P25 & Man                    & 23 & OSS Coder               & Mature project   & Video-conference \\ 
P26                     & Prefer not to disclose & 10                    & OSS Project Manager & Mature project       & Videoconference         \\ 
P27 & Woman                  & 10 & OSS Coder               & Mature project   & Video-conference \\ \hline
\end{tabular}
\end{table*}

==> Tables/Tables/demo_old.tex <==
\begin{table*}[htb]
\centering
\scriptsize
\caption{Demographics for the Interview Participants}
\label{tab:demo_old}
\begin{tabular}{|c|c|c|l|}
\hline
\textbf{Participant ID} & \textbf{Gender} & \textbf{Years in OSS} & \textbf{Main Role} \\\hline\hline
P1 & Woman & 6 & OSS Advocate \\\hline
P2 & Woman & 5 & OSS Coder  \\\hline
P3 & Woman & 13 & OSS Treasurer  \\\hline
P4 & Man & 9 & OSS System Admin  \\\hline
P5 & Prefer not to disclose & 7 & OSS Coder  \\\hline
P6 & Man & 5 & OSS Coder  \\\hline
P7 & Man & 12 & OSS Coder  \\\hline
P8 & Woman & 30 & OSS Strategist \\\hline
P9 & Man & 13 & OSS Advocate  \\\hline
P10 & Woman & 20 & OSS Advocate  \\\hline
P11 & Woman & 20 & OSS Writer \\\hline
P12 & Woman & 20 & OSS Advocate and Writer \\\hline
P13 & Woman & 7 & OSS Advocate \\\hline
P14 & Woman & 20 & OSS License Manager \\\hline
P15 & Woman & 15 & OSS Advocate \\\hline
P16 & Woman & 10 & OSS Advocate \\\hline
P17 & Woman & 5 & OSS Project Manager \\\hline
P18 & Man & 8 & OSS Coder \\\hline
P19 & Man & 8 & OSS Coder \\\hline
P20 & Man & 5 & OSS Coder \\\hline
P21 & Man & 15 & OSS Coder \\\hline
P22 & Man & 10 & OSS Advocate \\\hline
P23 & Man & 7 & OSS Coder \\\hline
P24 & Man & 20 & OSS Coder \\\hline
P25 & Man & 23 & OSS Coder \\\hline
P26 & Prefer not to disclose & 10 & OSS Project Manager \\\hline
P27 & Woman & 10 & OSS Coder \\\hline
\end{tabular}
\end{table*}

==> Tables/Tables/survey_demo.tex <==
\begin{table*}[htb]
\centering
\caption{Demographics for the Survey Respondents}
\label{tab:survey_demo}
\begin{tabular}{c|c|ccc|c|c}
\cline{1-3}\cline{5-7}
\cellcolor{gray!35}\textbf{Role} & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}  & \multirow{15}{*}{} & \cellcolor{gray!35}\textbf{Country of Residence} & \cellcolor{gray!35}\textbf{\#} & \cellcolor{gray!35}\textbf{\%}\\\cline{1-3}\cline{5-7}
Coder              & 163 & 84,46\% &                    & Germany              & 89 & 46,11\% \\
Non-Coder          & 30  & 15,54\% &                    & USA                  & 59 & 30,57\% \\\cline{1-3}
\multicolumn{3}{l}{}               &                    & Netherlands          & 12 & 6,22\%  \\\cline{1-3}
\cellcolor{gray!35}\textbf{Gender}             & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}      &                    & Brazil               & 9  & 4,66\%  \\\cline{1-3}
Men                & 165 & 85,49\% &                    & Others               & 23 & 11,92\% \\
Women              & 16  & 8,29\%  &                    & Did not answer       & 1  & 0,52\%  \\\cline{5-7}
Non-Binary         & 2   & 1,04\%  &\multicolumn{1}{l}{}& \multicolumn{3}{l}{}                \\\cline{5-7}
Did not answer     & 10  & 5,18\%  &                    & \cellcolor{gray!35}\textbf{Age}  & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}      \\\cline{1-3}\cline{5-7}
\multicolumn{3}{l}{}               &                    & 24 or less           & 30 & 15,54\% \\\cline{1-3}
\cellcolor{gray!35}\textbf{Financial Relation} & \cellcolor{gray!35}\textbf{\#}  & \cellcolor{gray!35}\textbf{\%}       &                    & 25-34                & 60 & 31,09\% \\
Paid               & 36  & 18,65\% &                    & 35-44                & 59 & 30,57\% \\
Unpaid             & 137 & 70,98\% &                    & 45-54                & 27 & 13,99\% \\
Partially Paid     & 16  & 8,29\%  &                    & 55 or more           & 10 & 5,18\%  \\
Did not answer     & 4   & 2,07\%  &                    & Did not answer       & 7  & 3,63\% \\\cline{1-3}\cline{5-7}
\end{tabular}
\end{table*}

==> Tables/demographics_after_before_OLD.tex <==
\begin{table*}[htb]
\centering
\scriptsize
\caption{Number of individuals who Started$\rightarrow$Continued because of each motivation by personal characteristics **.}
\label{tab:demographics_before_after}
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r}
\hline
\toprule
\textbf{Demographics / Motivations}                          & \textbf{Altruism} & \textbf{Career}  & \textbf{Enjoy./Fun} & \textbf{Gift/Recip.} & \textbf{Ideology} & \textbf{Kinship} & \textbf{Learning} & \textbf{Own-use} & \textbf{Pay}     & \textbf{Reputation} \\ \hline
  \midrule
  
Gender:Man (n=196)                                       & \cellcolor{gray!25}  34$\rightarrow$48     &  \cellcolor{gray!25} 9$\rightarrow$16   & \cellcolor{gray!25} 13$\rightarrow$40     & \cellcolor{gray!25} 23$\rightarrow$29       & \cellcolor{red!25}22$\rightarrow$14    & \cellcolor{gray!25} 6$\rightarrow$16    & 33$\rightarrow$40    & 50$\rightarrow$43   & 24$\rightarrow$28 &  \cellcolor{gray!25} 7$\rightarrow$19       \\
Gender:Woman (n=18)                                     & 0$\rightarrow$4  \cellcolor{gray!25}  &  0$\rightarrow$2    & 0$\rightarrow$1       & \cellcolor{gray!25} 1$\rightarrow$7         & 2$\rightarrow$1      &  0$\rightarrow$2     & 2$\rightarrow$3      & \cellcolor{red!25} 6$\rightarrow$1     & 2$\rightarrow$2   & 0$\rightarrow$1        \\
\toprule
OSS Exp:High(\textgreater{}=15) (n=65)              & \cellcolor{gray!25} 10$\rightarrow$22    & 2$\rightarrow$1    & 6$\rightarrow$9       & 8$\rightarrow$11        & 10$\rightarrow$8     & 3$\rightarrow$4     & 7$\rightarrow$5      & \cellcolor{red!25} 17$\rightarrow$11   & \cellcolor{gray!25} 5$\rightarrow$16  & 4$\rightarrow$5        \\
OSS Exp:Medium(\textgreater{}3\&\textless{}15) (n=98) & 22$\rightarrow$27    & 3$\rightarrow$5    & \cellcolor{gray!25} 2$\rightarrow$16      & \cellcolor{gray!25} 12$\rightarrow$16       & \cellcolor{red!25} 13$\rightarrow$9     & \cellcolor{gray!25} 2$\rightarrow$6     & 15$\rightarrow$15    & \cellcolor{red!25} 25$\rightarrow$21   & 11$\rightarrow$13 & \cellcolor{gray!25} 1$\rightarrow$9        \\
OSS Exp:Low(\textless{}=3) (n=63)                   &  6$\rightarrow$5   & \cellcolor{gray!25} 4$\rightarrow$12   & \cellcolor{gray!25} 6$\rightarrow$19      & \cellcolor{gray!25} 6$\rightarrow$11        & 2$\rightarrow$2      & \cellcolor{gray!25} 2$\rightarrow$10    & \cellcolor{gray!25} 15$\rightarrow$24    & \cellcolor{red!25} 18$\rightarrow$12   & 7$\rightarrow$4   & \cellcolor{gray!25} 2$\rightarrow$6        \\
\toprule
Age:(\textgreater{}=35 yrs) (n=112)                     & \cellcolor{gray!25} 19$\rightarrow$35    &   3$\rightarrow$6    & \cellcolor{gray!25}9$\rightarrow$16      & 15$\rightarrow$16       & 13$\rightarrow$10    & 5$\rightarrow$8     & 14$\rightarrow$12    & \cellcolor{red!25} 24$\rightarrow$18   & \cellcolor{gray!25} 17$\rightarrow$24 & \cellcolor{gray!25} 5$\rightarrow$11       \\
Age:(\textless{}35 yrs) (n=113)                       & 17$\rightarrow$17    & \cellcolor{gray!25} 6$\rightarrow$12   &\cellcolor{gray!25} 6$\rightarrow$27      & \cellcolor{gray!25} 11$\rightarrow$21       & 12$\rightarrow$9     & \cellcolor{gray!25}  2$\rightarrow$12    & \cellcolor{gray!25} 23$\rightarrow$32    & \cellcolor{red!25} 35$\rightarrow$26   & 9$\rightarrow$9   & \cellcolor{gray!25} 2$\rightarrow$9        \\
\toprule
Role:Coder (n=193)                                       & \cellcolor{gray!25} 30$\rightarrow$41    & \cellcolor{gray!25} 9$\rightarrow$17   & \cellcolor{gray!25} 15$\rightarrow$43     & \cellcolor{gray!25} 22$\rightarrow$30       & \cellcolor{red!25} 20$\rightarrow$13     & \cellcolor{gray!25} 4$\rightarrow$17     & \cellcolor{gray!25} 32$\rightarrow$40    & \cellcolor{red!25} 56$\rightarrow$41   &  \cellcolor{gray!25} 23$\rightarrow$30 & \cellcolor{gray!25} 6$\rightarrow$19       \\
Role:Non-Coder (n=45)                                   & \cellcolor{gray!25} 8$\rightarrow$15    &  0$\rightarrow$2    &  3$\rightarrow$3      & 6$\rightarrow$9       & 7$\rightarrow$7    &  3$\rightarrow$4    &  8$\rightarrow$10    & 7$\rightarrow$6   &  5$\rightarrow$6 & 2$\rightarrow$4       \\
\toprule
Residence:North America (n=70)                           & \cellcolor{gray!25} 13$\rightarrow$20    & 2$\rightarrow$5    & \cellcolor{gray!25} 2$\rightarrow$10      & \cellcolor{gray!25}6$\rightarrow$12        & 9$\rightarrow$6      & 3$\rightarrow$6     & 11$\rightarrow$8     & \cellcolor{red!25} 17$\rightarrow$13   & \cellcolor{gray!25} 11$\rightarrow$15 & 3$\rightarrow$5        \\
Residence:South America (n=25)                             & 4$\rightarrow$5      & 1$\rightarrow$2    & 1$\rightarrow$3       & 4$\rightarrow$5         & 3$\rightarrow$4      & 0$\rightarrow$1     & \cellcolor{gray!25} 3$\rightarrow$7      & 6$\rightarrow$5     & 3$\rightarrow$2   & 1$\rightarrow$3        \\
Residence:Europe (n=100)                                   & 18$\rightarrow$22    & 4$\rightarrow$7    & \cellcolor{gray!25} 10$\rightarrow$21     & 14$\rightarrow$17       & 9$\rightarrow$7      & \cellcolor{gray!25}  3$\rightarrow$9     & 16$\rightarrow$17    & \cellcolor{red!25} 32$\rightarrow$23   & \cellcolor{gray!25} 9$\rightarrow$15  & \cellcolor{gray!25} 3$\rightarrow$8        \\

%Country:Africa (n=2)                                   & 0$\rightarrow$0      & 0$\rightarrow$0    & 1$\rightarrow$1       & 1$\rightarrow$1         & 0$\rightarrow$0      & 0$\rightarrow$0     & 1$\rightarrow$1      & 0$\rightarrow$0     & 0$\rightarrow$0   & 0$\rightarrow$0        \\
%Country:Asia (n=16)                                     & \cellcolor{gray!25} 1$\rightarrow$3      & \cellcolor{gray!25} 2$\rightarrow$4    & \cellcolor{gray!25} 1$\rightarrow$6       & \cellcolor{gray!25} 0$\rightarrow$2         & \cellcolor{gray!25} 2$\rightarrow$0      & \cellcolor{gray!25} 0$\rightarrow$4     & \cellcolor{gray!25} 4$\rightarrow$8      & \cellcolor{red!25} 2$\rightarrow$0     &  \cellcolor{gray!25} 1$\rightarrow$0   &  \cellcolor{gray!25} 0$\rightarrow$2        \\
%Country:Oceania (n=7)                                 & \cellcolor{red!25} 2$\rightarrow$1      & 0$\rightarrow$0    & 0$\rightarrow$0       & 1$\rightarrow$1         & \cellcolor{gray!25} 1$\rightarrow$0      & 1$\rightarrow$0     & \cellcolor{gray!25} 1$\rightarrow$3      & \cellcolor{red!25} 2$\rightarrow$1     & \cellcolor{gray!25} 0$\rightarrow$1   & 0$\rightarrow$0     \\


\bottomrule
\end{tabular}

\resizebox{\textwidth}{!}{%
%\begin{tabularx}{\linewidth}{lX}
\begin{tabularx}{\linewidth}{@{}XXX@{}}
\\
** The table presents the number of respondents whose motivation to start (before the arrow) and to continue (after the arrow) fell into each motivation category.  We excluded from the table the GSoC and coursework categories due to the limited number of respondents.  We also excluded the continents and genders for which we had few responses. We highlight in gray/red those cases in which we observed an increase/decrease of at least 25\% when comparing the second number (motivation to continue) in relation to the first (motivation to start) and at least 3 individuals.
\end{tabularx}
}

\end{table*}






==> Tables/demographics_coding.tex <==
\begin{table*}[!h]
\centering
\scriptsize
\caption{Motivations by Demographics}
\label{tab:demographics}
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline

\multirow{2}{*}{\textbf{Motivations / Demographics}}         & \multicolumn{2}{l|}{\textbf{Altruism}} & \multicolumn{2}{l|}{\textbf{Career}} & \multicolumn{2}{l|}{\textbf{Enjoyment and fun}} & \multicolumn{2}{l|}{\textbf{Gift economy/Reciprocity}} & \multicolumn{2}{l|}{\textbf{Ideology}} & \multicolumn{2}{l|}{\textbf{Kinship}} & \multicolumn{2}{l|}{\textbf{Learning}} & \multicolumn{2}{l|}{\textbf{Own-use}} & \multicolumn{2}{l|}{\textbf{Pay}} & \multicolumn{2}{l|}{\textbf{Reputation}} \\ \cline{2-21} 
                                                    & before        & after         & before       & after        & before             & after             & before                & after                 & before        & after         & before        & after        & before        & after         & before        & after        & before      & after      & before         & after          \\ \hline
                                                    \toprule
Gender:Man                                          & 3.57\%        & 24.49\%       & 4.59\%       & 8.16\%       & 6.63\%             & 20.41\%           & 11.73\%               & 14.80\%               & 11.22\%       & 7.14\%        & 3.06\%        & 8.16\%       & 16.84\%       & 20.41\%       & 25.51\%       & 21.94\%      & 12.24\%     & 14.29\%    & 3.57\%         & 9.69\%         \\ \hline
Gender:Woman                                        & 0.00\%        & 22.22\%       & 0.00\%       & 11.11\%      & 0.00\%             & 5.56\%            & 5.56\%                & 38.89\%               & 11.11\%       & 5.56\%        & 0.00\%        & 11.11\%      & 11.11\%       & 16.67\%       & 33.33\%       & 5.56\%       & 11.11\%     & 11.11\%    & 0.00\%         & 5.56\%         \\ \hline
Experience:Mostly(\textgreater{}=15)                & 15.38\%       & 33.85\%       & 3.08\%       & 1.54\%       & 9.23\%             & 13.85\%           & 12.31\%               & 16.92\%               & 15.38\%       & 12.31\%       & 4.62\%        & 6.15\%       & 10.77\%       & 7.69\%        & 26.15\%       & 16.92\%      & 7.69\%      & 24.62\%    & 6.15\%         & 7.69\%         \\ \hline
Experience:Normal(\textgreater{}3 \& \textless{}15) & 22.45\%       & 27.55\%       & 3.06\%       & 5.10\%       & 2.04\%             & 16.33\%           & 12.24\%               & 16.33\%               & 13.27\%       & 9.18\%        & 2.04\%        & 6.12\%       & 15.31\%       & 15.31\%       & 25.51\%       & 21.43\%      & 11.22\%     & 13.27\%    & 1.02\%         & 9.18\%         \\ \hline
Experience:Less(\textless{}=3)                      & 9.52\%        & 7.94\%        & 6.35\%       & 19.05\%      & 9.52\%             & 30.16\%           & 9.52\%                & 17.46\%               & 3.17\%        & 3.17\%        & 3.17\%        & 15.87\%      & 23.81\%       & 38.10\%       & 28.57\%       & 19.05\%      & 11.11\%     & 6.35\%     & 3.17\%         & 9.52\%         \\ \hline
Age:Oldest(\textgreater{}=35)                       & 16.96\%       & 31.25\%       & 2.68\%       & 5.36\%       & 8.04\%             & 14.29\%           & 13.39\%               & 14.29\%               & 11.61\%       & 8.93\%        & 4.46\%        & 7.14\%       & 12.50\%       & 10.71\%       & 21.43\%       & 16.07\%      & 15.18\%     & 21.43\%    & 4.46\%         & 9.82\%         \\ \hline
Age:Younger(\textless{}35)                          & 15.04\%       & 15.04\%       & 5.31\%       & 10.62\%      & 5.31\%             & 23.89\%           & 9.73\%                & 18.58\%               & 10.62\%       & 7.96\%        & 1.77\%        & 10.62\%      & 20.35\%       & 28.32\%       & 30.97\%       & 23.01\%      & 7.96\%      & 7.96\%     & 1.77\%         & 7.96\%         \\ \hline
Role:Coder                                          & 17.73\%       & 21.99\%       & 6.38\%       & 8.51\%       & 8.51\%             & 23.40\%           & 10.64\%               & 17.73\%               & 9.22\%        & 5.67\%        & 2.13\%        & 5.67\%       & 19.15\%       & 21.28\%       & 28.37\%       & 18.44\%      & 12.06\%     & 14.89\%    & 2.13\%         & 8.51\%         \\ \hline
Role:Non-Coder                                      & 13.40\%       & 25.77\%       & 0.00\%       & 7.22\%       & 6.19\%             & 13.40\%           & 13.40\%               & 15.46\%               & 14.43\%       & 12.37\%       & 4.12\%        & 13.40\%      & 13.40\%       & 20.62\%       & 23.71\%       & 21.65\%      & 11.34\%     & 15.46\%    & 5.15\%         & 11.34\%        \\ \hline
Continent:NorthAmerica                              & 18.57\%       & 28.57\%       & 2.86\%       & 7.14\%       & 2.86\%             & 14.29\%           & 8.57\%                & 17.14\%               & 12.86\%       & 8.57\%        & 4.29\%        & 8.57\%       & 15.71\%       & 11.43\%       & 24.29\%       & 18.57\%      & 15.71\%     & 21.43\%    & 4.29\%         & 7.14\%         \\ \hline
Country:SouthAmerica                                & 16.00\%       & 20.00\%       & 4.00\%       & 8.00\%       & 4.00\%             & 12.00\%           & 16.00\%               & 20.00\%               & 12.00\%       & 16.00\%       & 0.00\%        & 4.00\%       & 12.00\%       & 28.00\%       & 24.00\%       & 20.00\%      & 12.00\%     & 8.00\%     & 4.00\%         & 12.00\%        \\ \hline
Country:Europe                                      & 18.00\%       & 22.00\%       & 4.00\%       & 7.00\%       & 10.00\%            & 21.00\%           & 14.00\%               & 17.00\%               & 9.00\%        & 7.00\%        & 3.00\%        & 9.00\%       & 16.00\%       & 17.00\%       & 32.00\%       & 23.00\%      & 9.00\%      & 15.00\%    & 3.00\%         & 8.00\%         \\ \hline
Country:Africa                                      & 0.00\%        & 0.00\%        & 0.00\%       & 0.00\%       & 50.00\%            & 50.00\%           & 50.00\%               & 50.00\%               & 0.00\%        & 0.00\%        & 0.00\%        & 0.00\%       & 50.00\%       & 50.00\%       & 0.00\%        & 0.00\%       & 0.00\%      & 0.00\%     & 0.00\%         & 0.00\%         \\ \hline
Country:Asia                                        & 6.25\%        & 18.75\%       & 12.50\%      & 25.00\%      & 6.25\%             & 37.50\%           & 0.00\%                & 12.50\%               & 12.50\%       & 0.00\%        & 0.00\%        & 25.00\%      & 25.00\%       & 50.00\%       & 12.50\%       & 0.00\%       & 6.25\%      & 0.00\%     & 0.00\%         & 12.50\%        \\ \hline
Country:Oceania                                     & 28.57\%       & 14.29\%       & 0.00\%       & 0.00\%       & 0.00\%             & 0.00\%            & 14.29\%               & 14.29\%               & 14.29\%       & 0.00\%        & 14.29\%       & 0.00\%       & 14.29\%       & 42.86\%       & 28.57\%       & 14.29\%      & 0.00\%      & 14.29\%    & 0.00\%         & 0.00\%         \\ \hline
\end{tabular}
\end{table*}

==> Tables/demographics_difference.tex <==
\begin{table*}[htb]
\centering
\scriptsize
\caption{Motivations Migration by Demographics}
\label{tab:demographics_difference}
\begin{tabular}{l|l|l|l|l|l|l|l|l|l|l}
\hline
\textbf{Demographics / Motivations}                          & \textbf{Altruism} & \textbf{Career}  & \textbf{Enjoy./Fun} & \textbf{Gift/Recip.} & \textbf{Ideology} & \textbf{Kinship} & \textbf{Learning} & \textbf{Own-use} & \textbf{Pay}     & \textbf{Reputation} \\ \hline
  \toprule
Gender:Man (n=196)                                         & 34/48/20.9\% \cellcolor{gray!25}  & 3.57\%  & 13.78\% \cellcolor{gray!25}           & 3.06\%                   & 4.08\%   & 5.10\%  & 3.57\%   & 3.57\%  & 2.04\%  & 6.12\%     \\ \hline
Gender:Woman (n=18)                                       & 22.22\% \cellcolor{gray!25}  & 11.11\% \cellcolor{gray!25} & 5.56\%            & 33.33\%   \cellcolor{gray!25}                & 5.56\%   & 11.11\%  \cellcolor{gray!25} & 5.56\%   & 27.78\%  \cellcolor{gray!25} & 0.00\%  & 5.56\%     \\ \hline
Experience:Mostly(\textgreater{}=15) (n=65)                & 18.46\% \cellcolor{gray!25}  & 1.54\%  & 4.62\%            & 4.62\%                   & 3.08\%   & 1.54\%  & 3.08\%   & 9.23\%  & 16.92\% \cellcolor{gray!25} & 1.54\%     \\ \hline
Experience:Normal(\textgreater{}3 \& \textless{}15) (n=98) & 5.10\%   & 2.04\%  & 14.29\%  \cellcolor{gray!25}          & 4.08\%                   & 4.08\%   & 4.08\%  & 0.00\%   & 4.08\%  & 2.04\%  & 8.16\%     \\ \hline
Experience:Less(\textless{}=3) (n=63)                     & 1.59\%   & 12.70\% \cellcolor{gray!25}  & 20.63\%  \cellcolor{gray!25}  & 7.94\%                   & 0.00\%   & 12.70\% \cellcolor{gray!25} & 14.29\% \cellcolor{gray!25}  & 9.52\%  & 4.76\%  & 6.35\%     \\ \hline
Age:Oldest(\textgreater{}=35) (n=112)                     & 14.29\% \cellcolor{gray!25}  & 2.68\%  & 6.25\%            & 0.89\%                   & 2.68\%   & 2.68\%  & 1.79\%   & 5.36\%  & 6.25\%  & 5.36\%     \\ \hline
Age:Younger(\textless{}35) (n=113)                         & 0.00\%   & 5.31\%  & 18.58\%   \cellcolor{gray!25} & 8.85\%                   & 2.65\%   & 8.85\%  & 7.96\%   & 7.96\%  & 0.00\%  & 6.19\%     \\ \hline
Role:Coder  (n=141)                                       & 4.26\%   & 2.13\%  & 14.89\%           & 7.09\%                   & 3.55\%   & 3.55\%  & 2.13\%   & 9.93\%  & 2.84\%  & 6.38\%     \\ \hline
Role:Non-Coder   (n=97)                                   & 12.37\% \cellcolor{gray!25}  & 7.22\%  & 7.22\%            & 2.06\%                   & 2.06\%   & 9.28\%  & 7.22\%   & 2.06\%  & 4.12\%  & 6.19\%     \\ \hline
Continent:NorthAmerica  (n=70)                            & 10.00\% \cellcolor{gray!25}   & 4.29\%  & 11.43\% \cellcolor{gray!25}           & 8.57\%                   & 4.29\%   & 4.29\%  & 4.29\%   & 5.71\%  & 5.71\%  & 2.86\%     \\ \hline
Country:SouthAmerica (n=25)                           & 4.00\%   & 4.00\%  & 8.00\%            & 4.00\%                   & 4.00\%   & 4.00\%  & 16.00\% \cellcolor{gray!25}  & 4.00\%  & 4.00\%  & 8.00\%     \\ \hline
Country:Europe (n=100)                                     & 4.00\%   & 3.00\%  & 11.00\%  \cellcolor{gray!25}          & 3.00\%   & 2.00\%   & 6.00\%  & 1.00\%   & 9.00\%  & 6.00\%  & 5.00\%     \\ \hline
Country:Africa  (n=2)                                   & 0.00\%   & 0.00\%  & 0.00\%            & 0.00\%                   & 0.00\%   & 0.00\%  & 0.00\%   & 0.00\%  & 0.00\%  & 0.00\%     \\ \hline
Country:Asia  (n=16)                                      & 12.50\%  \cellcolor{gray!25}  & 12.50\% \cellcolor{gray!25}  & 31.25\% \cellcolor{gray!25}           & 12.50\%  \cellcolor{gray!25}                 & 12.50\% \cellcolor{gray!25}  & 25.00\% \cellcolor{gray!25} & 25.00\% \cellcolor{gray!25}  & 12.50\% \cellcolor{gray!25}  & 6.25\%  & 12.50\% \cellcolor{gray!25}     \\ \hline
Country:Oceania  (n=7)                                    & 14.29\%  \cellcolor{gray!25}  & 0.00\%  & 0.00\%            & 0.00\%                   & 14.29\% \cellcolor{gray!25}  & 14.29\% \cellcolor{gray!25} & 28.57\% \cellcolor{gray!25}  & 14.29\% \cellcolor{gray!25}  & 14.29\% \cellcolor{gray!25}  & 0.00\%     \\ \hline
\end{tabular}
\end{table*}




==> Tables/pairs.tex <==
\begin{table}[t]
	\centering
	\caption{A list of TOP-10 pairwise motivations migration.}
	\label{tab:pairs_of_motivations}	
	    \begin{tabular}{l c l}
	    \toprule
         TOP Migration Flow Patterns & \# Mentions \\
        \hline        
        \midrule
        Learning $\Rightarrow$ Gift economy/Reciprocity & 14 \\
        Own-use $\Rightarrow$ Altruism & 13
        \\
        Own-use $\Rightarrow$ Learning & 13
        \\
        Own-use $\Rightarrow$ Enjoyment and fun & 12
        \\
        Gift economy/Reciprocity $\Rightarrow$ Altruism & 11
        \\
        Learning $\Rightarrow$ Altruism & 11
        \\
        Own-use $\Rightarrow$ Gift economy/Reciprocity & 10
        \\
        Learning $\Rightarrow$ Own-use & 9
        \\
        Learning $\Rightarrow$ Enjoyment and fun & 8
        \\
        Altruism $\Rightarrow$ Gift economy/Reciprocity & 8
        \\
        Altruism $\Rightarrow$ Learning & 8
        \\
        Own-use $\Rightarrow$ Pay & 8
        \\
        \hline
    \end{tabular}
\end{table}

==> Tables/previous_comparison.tex <==
\begin{table*}[htb]
\centering
\scriptsize
\caption{The previous more cited previous surveys about motivations of OSS contributors}
\label{tab:comparison}
\begin{tabular}{ccccc}
\hline
\toprule
                                                                           & Ghosh et. al \cite{ghosh2002free}  & Hars and Ou \cite{harsworking}   & Lakhani and Wolf \cite{lakhani2003hackers} & Hertel et.al \cite{hertel2003motivation} \\ \hline
\midrule

\begin{tabular}[c]{@{}c@{}}Number of \\ Responses\end{tabular}             & 2784          & 81            & 684              & 141          \\ \hline

\begin{tabular}[c]{@{}c@{}}Number of \\ Different \\ Projects\end{tabular} & Not mentioned & Not mentioned & 287              & 1 (Linux)    \\ \hline
\begin{tabular}[c]{@{}c@{}}Distribution \\ Method\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Questionnaire posted\\  to few OSS communities\\  and then distributed \\ by OSS developers\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}E-mails to OSS \\ contributors from \\ discussion lists \\ and newsgroups\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}E-mails to OSS \\ contributors listed\\  as official developers\\  at SourceForge.net\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Announcements\\  on Linux mailing-lists\\ inviting to contribute \\ and then to answer\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Categories \\ to Organize \\ Motivations\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Intrinsic \\ Motivations \\ (Enjoyment and \\ Obligation/Community)\\ Economic/Extrinsic \\ Motivations\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Internal\\ External\\ Future Rewards\\ Personal Need\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Reasons to Join OSS\\ Reasons to Stay in OSS\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Specific identification\\ Norm-oriented motives\\ Pragmatic motives\\ Social/political motives\\ Hedonistic motives\\ Time loss (rev. coding)\\ Hours/week spent \\ on Linux development\\ Willingness to be \\ involved in the future\end{tabular} \\ \hline
\end{tabular}
\end{table*}
